Diffusion Models Without Attention

In recent advancements in high-fidelity image generation, Denoising Diffusion Probabilistic Models (DDPMs) have emerged as a key player. However, their application at high resolutions presents significant computational challenges. Current methods, such as patchifying, expedite processes in UNet and Transformer architectures but at the expense of representational capacity. Addressing this, we introduce the Diffusion State Space Model (DiffuSSM), an architecture that supplants attention mechanisms with a more scalable state space model backbone. This approach effectively handles higher resolutions without resorting to global compression, thus preserving detailed image representation throughout the diffusion process. Our focus on FLOP-efficient architectures in diffusion training marks a significant step forward. Comprehensive evaluations on both ImageNet and LSUN datasets at two resolutions demonstrate that DiffuSSMs are on par or even outperform existing diffusion models with attention modules in FID and Inception Score metrics while significantly reducing total FLOP usage.

==> imagenet.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l|cc|ccccc}
\midrule
\midrule

\multicolumn{5}{l}{\textbf{ImageNet 256×256 Benchmark}} \\
\midrule
     Models  & Total & Total  & FID $\downarrow$ & sFID $\downarrow$& IS $\uparrow$& P $\uparrow$ & R $\uparrow$ \\
     & Images(M) & Gflops  &  &  &  &  &  \\
\midrule
BigGAN-deep~\citep{brock2018large} & -   & - & 6.95 &   7.36 &     171.40  &  0.87 &   0.28               \\
MaskGIT~\citep{chang2022maskgit} & 355  & -  &6.18  &  -  &  182.1  &  0.80 &   0.51               \\
StyleGAN-XL~\citep{sauer2022stylegan} & - & - &  \textbf{2.30}  &  4.02    & 265.12 &  0.78 &  0.53      \\
\midrule
ADM~\citep{dhariwal2021diffusion}  & 507 &  $5.68\times10^{12}$ &  10.94  &  6.02 &   100.98   &  0.69 &     0.63   \\
ADM-U~\citep{dhariwal2021diffusion}  & 507 &   $3.76\times10^{11}$  &     7.49  & 5.13 &   127.49   &  0.72 &     0.63   \\
\arrayrulecolor{mylightgray} % Set \hline color to gray
\hline
CDM~\citep{ho2022cascaded} & - & - & 4.88  &   -  & 158.71  &   -  &     -       \\
\arrayrulecolor{mylightgray} % Set \hline color to gray
\hline
\arrayrulecolor{mylightgray} % Set \hline color to gray
\hline
LDM-8~\citep{rombach2022high}  & 307 & $1.75\times10^{10}$ & 15.51   &  - &   79.03    & 0.65  &  0.63        \\
LDM-4~\citep{rombach2022high} &  213 & $2.22\times10^{10}$ &  10.56   &  - &    103.49    & 0.71  &  0.62        \\
% DiT-XL/2 & 602 & $7.10\times10^{10}$ &  10.67   &  -   &  -    & - &   -       \\
DiT-XL/2~\citep{peebles2022scalable} & 1792 &  $2.13\times10^{11}$  & 9.62  &  6.85   &  121.50    & 0.67 &   0.67       \\
\arrayrulecolor{black}
%\midrule
% \textbf{\model-XL}  & 338 & $9.57\times10^{10}$ &  9.86  &  5.51 &   111.59   & 0.69    &  0.64       \\
\textbf{\model-XL}  & 660 & $1.85\times10^{11}$ &  \textbf{9.07}   &  5.52 &   118.32   & 0.69    &  0.64       \\
\midrule
\midrule
Classifier-free Guidance \\
\midrule
ADM-G  &  507 &  $5.68\times10^{11}$  & 4.59  &   5.25   & 186.70 & 0.82   &  0.52    \\
ADM-G, ADM-U  & 507 & $3.76\times10^{12}$ &  3.60  &   -   & 247.67 & 0.87   & 0.48       \\
LDM-8-G  & 307 & $1.75\times10^{10}$   &    7.76  & -   & 209.52    & 0.84 &  0.35    \\
LDM-4-G  &  213 &  $2.22\times10^{10}$  &  3.95 &   -   &   178.2 2 & 0.81   &  0.55      \\
U-ViT-H/2-G~\citep{bao2023all}  &  512  & $6.81\times10^{10} $& 2.29  &   -   & 247.67 & 0.87   & 0.48       \\
% DiT-XL/2(G-1.25) & 1792 &   $2.13\times10^{11}$ & 3.22 &  5.28     & 201.77  & 0.76  &  0.62   \\
DiT-XL/2-G  & 1792 &   $2.13\times10^{11}$  &  \textbf{2.27} &   4.60   & 278.24  & 0.83  &  0.57    \\
%\midrule
% \textbf{\model-XL}(G-1.5) &  338 & $9.57\times10^{10}$ & 2.91 &  4.55     & 247.84  & 0.76  &  0.62   \\
\textbf{\model-XL}-G &  660 &  $1.85\times10^{11}$  & 2.28 &  \textbf{4.49}     & 259.13  & 0.86  &  0.56    \\
\midrule
\midrule
\multicolumn{5}{l}{\textbf{ImageNet 512×512 Benchmark}} \\
\midrule
ADM &  1385  & $5.97\times 10^{11}$  & 23.24 &   10.19  & 58.06  &   0.73    &  0.60        \\
ADM-U & 1385 &  $3.9\times 10^{12}$  & 9.96 &   5.62   & 121.78  &   0.75   &  0.64       \\
ADM-G & 1385 & $5.97\times 10^{11}$   & 7.72    & 6.57   &  172.71    & 0.87  &   0.42    \\
ADM-G, ADM-U & 1385 &  $4.5\times 10^{12}$ &  3.85 &  5.86    & 221.72  & 0.84 &   0.53      \\
\arrayrulecolor{mylightgray} % Set \hline color to gray
\hline
U-ViT/2-G  & 512 &  $6.81\times 10^{10}$  &   4.05   & 8.44 &  261.13 &  0.84     & 0.48   \\
DiT-XL/2-G   & 768 & $4.03\times 10^{11}$ & \textbf{3.04} &   \textbf{5.02}   &  240.82 & 0.84  &0.54          \\
\arrayrulecolor{black} 
%\midrule
\textbf{\model-XL-G}  & 307  & $3.22\times 10^{11}$ &      &   &   &  &         \\
\hline
\end{tabular}
\caption{Class conditional image generation quality evaluation of \model and existing approaches
% (BigGAN-deep~\citep{brock2018large},
% MaskGIT~\citep{chang2022maskgit},
% StyleGAN-XL~\citep{sauer2022stylegan},
% ADM~\citep{dhariwal2021diffusion},
% LDM-8~\citep{rombach2022high},
% DiT-XL/2~\citep{peebles2022scalable},
% CDM~\citep{ho2022cascaded}, U-Vit~\citep{bao2023all}) 
on ImageNet 256$\times$ 256. We took reported results from other papers with their $\#$ trained images. We calculated the Total images by training steps $\times$ batch size as reported in their paper, and total Gflops by Total Images $\times$ GFlops/Image. P refers to Precision and R refers to Recall. $-G$ denotes
the results with classifier-free guidance. }
\end{table*}

==> model_old.tex <==
\section{Fine-Grained Diffusion with SSMs}

Our goal is to produce a diffusion architecture that works on the flattened representation. 



\subsection{State Space Models}
%1. What's SSM?
%2. SSM can be used for discrete time series
%3. We have used S4D for the simplicity of the paper
%More details can be found in the appendix

SSM-based neural networks provide an alternative architecture for transforming discrete sequences, which provides an alternative approach to sequence modeling in neural networks without the quadratic computational cost of attention. 

Mathematically, SSMs map a continuous input $u(t)$ to a output $y(t)$ by the following differential equation:

\begin{align*}
    x'(t) = \boldsymbol{A}x(t) + \boldsymbol{B}u(t),\ \ \ 
    y(t) = \boldsymbol{C}x(t) + \boldsymbol{D}u(t).
\end{align*}
\noindent Where $x(t) \in \mathbb{R}^{N}$ is a continuous-time state vector, $x'(t)$ is its derivative, and the equation is parameterized by $\boldsymbol{A} \in \mathbb{R}^{N\times N}, \boldsymbol{B}\in \mathbb{R}^{N \times 1}, \boldsymbol{C} \in \mathbb{R}^{1 \times N}, \boldsymbol{D} \in \mathbb{R}^{1\times 1}$.

We can apply a $\Delta t$ time scalar to discrete the SSMs parameters when applying to a discrete sequence. 
\begin{align*}
x_{k} = \boldsymbol{\overline{A}} x_{k-1} + \boldsymbol{\overline{B}} u_k,  \ \ \ 
y_k = \boldsymbol{\overline{C}} x_k + \boldsymbol{\overline{D}}  u_k. 
\end{align*}
Where $\boldsymbol{\overline{A}},\boldsymbol{\overline{B}},\boldsymbol{\overline{C}},\boldsymbol{\overline{D}}$ are functions of the original parameters and a discretization rate.

\textbf{Bi-directional SSMs}.
The bidirectional S4 state-space model is a simple variant of the S4 state-space model that can be used for non-autoregressive tasks. It works by passing the input sequence through two separate S4 layers, one in the forward direction and one in the backward direction. The outputs of the two S4 layers are then concatenated and passed through a positionwise linear layer. In this paper, we used bi-directional SSM as our major backbone component.  


\paragraph{Variants of SSMs}\citet{gu2020hippo, gu2021efficiently} demonstrate an effective  
approach for using SSMs in neural networks. They develop a parameterization 
of $\boldsymbol{A}$, known as HiPPO, yielding a stable and efficient architecture known as S4. This retains the SSM ability to model long-term sequences while being more efficient than RNNs to train. 
Recently, researchers~\citep{gu2022parameterization, gupta2022diagonal} have proposed simplified diagonalized versions of S4, which achieve comparable results with a simpler approximation of the original parameterization. 
In this paper, we chose S4D\citep{gu2022parameterization} as the major backbone. 


% \srush{Need to remind the reader of a) what the goals of this work are, b) connect them to the specific decisions -> remove compression/switch to more efficient routing / down-up sampling} 

% \subsection{Flatten Sequence}

% Taking the advantage of computational efficiency of SSMs, our approach gets rid of patching and considers the case where $p=1$, the input image $x \in \mathbb{R}^{H\times W \times C}$ is not split into patches. Instead, each pixel is treated as an individual input and flattened into a  full spatial resolution, C-dimension:
% $\mathbf{x}_i = \text{flatten}(x_i) \in \mathbb{R}^d, \mathbf{X} = [\mathbf{x}_1, ..., \mathbf{x}_{L}], \text{where}~\mathbf{X} \in \mathbb{R}^{L\times d},~\text{and}~L=H\times W$. 





\subsection{\model block Architecutre}\label{sec:arch}

Following flattening, the input image representations are fed into a sequence of  \model blocks.

As shown in Figure \ref{fig:models}

\begin{figure*}[t]\label{fig:models}\vspace{-3em}
    \centering    
    \includegraphics[width=.5\linewidth]{Figures/model_architecture.pdf}
\caption{\model Block}
\end{figure*}

% \subsection{Hourglass FFN}
% Our analysis has revealed that a significant portion of the FLOPs are expended in the Feed forward(FNN) layers. However, it is the SSM core that carries out the most critical computation, where a more fine-grained representation might assist in preserving the most valuable information. Consequently, we proposed the `hourglass' architecture. Given the flattened representation $\mathbf{X}  \in \mathbb{R}^{L \times d}$, these designs aim to minimize the length of $\mathbf{X}$ to a fraction $m$ of $L$ in the FFN or dense layers, while subsequently restoring $\mathbf{X}$ to its full length in the fine-grained SSM core.

% The process of convolution sampling introduces trainable parameters with a fractional factor up-down sampling ratio $m$. Prior to directing the flattened noise into the fine-grained SSM core, we first apply downsampling to decrease the length of $\mathbf{X}$. Following the computation in the fine-grained SSM core, we then employ upsampling to restore the original length of $\mathbf{X}$ and do the down-sampling again to after leaving the fine-grained SSM core. 



% \subsection{\model Block}
% \na{Still editing}

% % \srush{at this point of the story you should have abstracted from image terminology "pixel" should just be math}
% % To simplify our discussion, we will consider only the pixel space $x \in \mathbb{R}^{H \times W \times C}$ for illustrative purposes. 
% The \model core block comprises two primary branches: the first one takes the flattened $\mathbf{X}$ as input, while the other two utilize a combination of the class label $\mathbf{y} \in \mathbb{R}^{\frac{L}{m} \times 1}$ and timestep $\mathbf{t} \in \mathbb{R}^{\frac{L}{m} \times 1}$, as illustrated in Figure \ref{fig:model:arch}. Let $\mathbf{X_j} \in \mathbb{R}^{\frac{L}{m}\times d}$ represent the flattened image input at the $j$-th layer.  

% At each layer of the \model Block, we initiate the layer normalization of $\mathbf{X}$, which can be expressed as $\mathbf{X} = \text{LayerNorm}(\mathbf{X_j} ) \in \mathbb{R}^{\frac{L}{m} \times d}$. Afterward, we apply the scale and shift module, adapting the strategy from the DiT\citep{peebles2022scalable} for better training purpose. 
% % For simplicity, we consider only the pixel space for illustration. The full core block consists of two major branches: one that accepts the input of flattened $\mathbf{X}$, and another that combines the class label $\mathbf{y} \in \mathbb{R}^{\frac{L}{m} \times 1}$ and timestep $\mathbf{t} \in \mathbb{R}^{\frac{L}{m} \times 1}$, as shown in Figure \ref{fig:architecture}(b). Let $\mathbf{X_j} \in \mathbb{R}^{C}$ represent the flattened image input at the $j$-th layer, where the channel dimension is $C$. We use the activation function GELU for $\sigma$. At each layer of the Core Block, we begin with layer normalization of $\mathbf{X}$, where $\mathbf{X} = \text{LayerNorm}(\mathbf{X_j}) \in \mathbb{R}^{\frac{L}{m} \times d}$.

% % \srush{this is details, should not be in the main methods section}

% % $\mathbf{X}  = \mathbf{X} \odot (1 + \gamma) + \beta  \in \mathbb{R}^{\frac{L}{m} \times d}$. 

% Next, we used the pair of up- and down-sampling modules sandwiched on the fine-grained block. We used this pair to recover $\mathbf{X}$ to of high granularity. 


% % Following that, we pass $\mathbf{U}$ to a linear layer and use a gate mechanism to combine $U$ and $\mathbf{V}$. 

% % \begin{align*}
% %   & \mathbf{O} = \mathbf{W}_o (\mathbf{W}_{u_1}(\mathbf{U})\odot \mathbf{V}) && \in \mathbb{R}^{\frac{L}{m}\times d},\\
% % \end{align*}

% Finally, a gating mechanism with learnable parameters $\alpha$ that is initialized to 0 and applied before the residual connection: $\alpha = \textbf{adaLN}(t, y)~ \text{where}~ \text{init. } \alpha=0$ . 

% % \begin{align*}
% %    \mathbf{X}_{j+1} = \alpha \odot \mathbf{O} + \mathbf{X_{j}}  && \in \mathbb{R}^{\frac{L}{m} \times d} 
% % \end{align*} 
% % \subsection{Decoding}
% % \srush{if this isn't new move to experimental setup}

% % The input to our model is, for example, flattened representation $\mathbf{X}\in \mathbb{R}^{L \times d}$ of a spatial representation $x$ (e.g. of 256x256x3 images). After passing through DiSSM Blocks, our model uses a standard linear decoder to convert the sequence of image tokens back into the original spatial dimensions. Specifically, after the final DiSSM block, each token is linearly projected into each spatial point (e.g. where C is the number of channels). This is done for every token in the sequence. Each point is then rearranged back into its original spatial layout to produce the predicted noise and covariance, both of which have the same dimensions as the original input representation $x$.


==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


